Exploratory Experiments on Programming Autonomous Robots in Jadescript

This paper describes exploratory experiments to validate the possibility of programming autonomous robots using an agent-oriented programming language. Proper perception of the environment, by means of various types of sensors, and timely reaction to external events, by means of effective actuators, are essential to provide robots with a sufficient level of autonomy. The agent-oriented programming paradigm is relevant with this respect because it offers language-level abstractions to process events and to command actuators. A recent agent-oriented programming language called Jadescript is presented in this paper together with its new features specifically designed to handle events. Exploratory experiments on a simple case-study application are presented to show the validity of the proposed approach and to exemplify the use of the language to program autonomous robots.

==> eptcsdata.tex <==
\providecommand{\firstpage}{55}
\providecommand{\publicationstatus}{R.C. Cardoso, A. Ferrando, D. Briola, C. Menghi,\\ T. Ahlbrecht (Eds.): First Workshop on Agents and\\ Robots for reliable Engineered Autonomy 2020 (AREA'20).\\
EPTCS 319, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.319.5}{10.4204/EPTCS.319.5}}
\pdfoutput=1

